TimeRAF: Retrieval-Augmented Foundation model for Zero-shot Time Series Forecasting

Time series forecasting plays a crucial role in data mining, driving rapid advancements across numerous industries. With the emergence of large models, time series foundation models (TSFMs) have exhibited remarkable generalization capabilities, such as zero-shot learning, through large-scale pre-training. Meanwhile, Retrieval-Augmented Generation (RAG) methods have been widely employed to enhance the performance of foundation models on unseen data, allowing models to access to external knowledge. In this paper, we introduce TimeRAF, a Retrieval-Augmented Forecasting model that enhance zero-shot time series forecasting through retrieval-augmented techniques. We develop customized time series knowledge bases that are tailored to the specific forecasting tasks. TimeRAF employs an end-to-end learnable retriever to extract valuable information from the knowledge base. Additionally, we propose Channel Prompting for knowledge integration, which effectively extracts relevant information from the retrieved knowledge along the channel dimension. Extensive experiments demonstrate the effectiveness of our model, showing significant improvement across various domains and datasets.

==> comments.tex <==



3.3里面，training data和knowledge base之间是什么关系？training data应该包括ts和knowledge base吧，188行默认了knowledge base和ts是一样的？

183行，“knowledge base = ” 看着像伪代码。等号左边换成个字母，比如B？
188行equal proportion表意不清，谁和谁equal？ts和knowledge base equal还是knowledge base domain之间equal？

3.4第一段，一定要是external吗
206行，channel prompting加个粗体？

223是第一次出现candidate这个词吗，candidate是否需要解释一下，knowledge base里每一条就是一个candidate

**3.5节开头缺乏整体逻辑和思想的介绍。DPR是啥，我们做了啥
3.5.1第一段，why similarity score， why 点积。总起段落不是说一句话总结模结构，而是一句话总结模型设计思想
比如：knowledge retriever是一个encoder，他可以将输入的knowledge candidate的信息提取，得到一个新的emb，我们希望这个emb的特性是，不仅能包含知识，还得涵盖他对预测任务的帮助程度。接下来我们介绍如何设计encoder的结构及其训练目标。

================
4. Experiments

4.1 Experiment Setups
Datasets: Include a table for Dataset A (in bold).
Implementation Details
Baselines
Evaluation Metrics

4.2 Results on Full-shot and Zero-shot Forecasting
Full-shot: TimeRAF and TimeRAF_R.
Zero-shot: TimeRAF, TimeRAF_R, TimeRAF_D.

4.3 Ablation Studies
Effectiveness of the Retriever
Integration Techniques
Channel Prompting

4.4 Analysis
Choice of Knowledge Base: Discuss the sources and scale of the knowledge base used.
Influence of Candidate Numbers
Case Study


==================
第一段最后一句话，多加几个TS foundation model的引用，不能只引survey paper啊 
第三段末尾，说我们设计了xxx model，第四段说challenge，逻辑反了，应该先说challenge再说model
line 82, no simple
contribution这里和上一段重复太多了，而且格式看起来非常浪费篇幅。
intro写的还是内容太少了，最好再加一两段，比如1、2段之间，或者第二段以后再加一两段讨论
3.2问题定义读起来像是符号解释，通篇没提求什么样的model呢？且问题定义没提rag的部分呀，knowledge呢？

==========================
前两个自然段的逻辑不清晰
(1)TS popular -> need large amount historical labeled data -> zeroshot is demanding （TS backgound 介绍的太远了,怎么都从ARIMA开始了。。。且这段是说zeroshot这个task的意义，跟TS没啥关系呀）
(2)foundation models have good generalization abilities for zeroshot (跟TS还是没啥关系呀) 
(3)foundation model not generalize well（前一段刚说了 good generalization 啊，到底好不好嘛） -> need prior knowledge to enhance 

另一个逻辑
(1)[backgound of TS foundation model for zeroshot]TS task popular，but most traditional methods learn from single domain, small amount of data, uperbounded generalization ability. nowadays, foundation models rise to prominence, training in different domains with large scale data, enpower zeroshot ability, which evolving the landscape of xxx domains， TS foundation models also rise. rapidly advance TS forecasting and applied on zeroshot tasks.
(2)[background of RAG，可以抄https://arxiv.org/pdf/2202.01110 section 2.1] RAG is a popular technique facilitating foundation models in xxx domain. Some researchers suggest to endow models the capability to access 【external memory】 via some information retrieval techniques, so that they can acquire more information in the generation process.讲讲问题定义，举例一下text上的RAG。提出问题，TS+RAG是否会有效？

=====================
intro 第一段有一个失败引用



